Privacy-Enhancing Technologies for Financial Data Sharing

Today, financial institutions (FIs) store and share consumers' financial data for various reasons such as offering loans, processing payments, and protecting against fraud and financial crime. Such sharing of sensitive data have been subject to data breaches in the past decade. While some regulations (e.g., GDPR, FCRA, and CCPA) help to prevent institutions from freely sharing clients' sensitive information, some regulations (e.g., BSA 1970) require FIs to share certain financial data with government agencies to combat financial crime. This creates an inherent tension between the privacy and the integrity of financial transactions. In the past decade, significant progress has been made in building efficient privacy-enhancing technologies that allow computer systems and networks to validate encrypted data automatically. In this paper, we investigate some of these technologies to identify the benefits and limitations of each, in particular, for use in data sharing among FIs. As a case study, we look into the emerging area of Central Bank Digital Currencies (CBDCs) and how privacy-enhancing technologies can be integrated into the CBDC architecture. Our study, however, is not limited to CBDCs and can be applied to other financial scenarios with tokenized bank deposits such as cross-border payments, real-time settlements, and card payments.

==> flowchart.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,340); %set diagram left start at 0, and has height of 340

%Flowchart: Terminator [id:dp6605264728425754] 
\draw   (21.2,130) -- (68.8,130) .. controls (74.99,130) and (80,138.95) .. (80,150) .. controls (80,161.05) and (74.99,170) .. (68.8,170) -- (21.2,170) .. controls (15.01,170) and (10,161.05) .. (10,150) .. controls (10,138.95) and (15.01,130) .. (21.2,130) -- cycle ;
%Flowchart: Decision [id:dp8970830619395258] 
\draw   (165,130) -- (200,150) -- (165,170) -- (130,150) -- cycle ;
%Straight Lines [id:da28490178947827227] 
\draw    (42,240) -- (127,240) ;
\draw [shift={(130,240)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da6185911213522297] 
\draw    (165,130) -- (165,103) ;
\draw [shift={(165,100)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da8272384059239716] 
\draw    (525,170) -- (525,197) ;
\draw [shift={(525,200)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Flowchart: Decision [id:dp643006124052622] 
\draw   (165,60) -- (200,80) -- (165,100) -- (130,80) -- cycle ;
%Flowchart: Decision [id:dp20802608823846613] 
\draw   (285,130) -- (320,150) -- (285,170) -- (250,150) -- cycle ;
%Flowchart: Decision [id:dp6971121595251547] 
\draw   (405,130) -- (440,150) -- (405,170) -- (370,150) -- cycle ;
%Flowchart: Decision [id:dp8359785943335073] 
\draw   (525,130) -- (560,150) -- (525,170) -- (490,150) -- cycle ;
%Flowchart: Process [id:dp23759168548675957] 
\draw   (485.5,201) -- (565.5,201) -- (565.5,271) -- (485.5,271) -- cycle ;
%Flowchart: Process [id:dp656494867310959] 
\draw   (485,29.5) -- (565,29.5) -- (565,99.5) -- (485,99.5) -- cycle ;
%Flowchart: Terminator [id:dp16284309811356845] 
\draw   (597.2,130) -- (644.8,130) .. controls (650.99,130) and (656,138.95) .. (656,150) .. controls (656,161.05) and (650.99,170) .. (644.8,170) -- (597.2,170) .. controls (591.01,170) and (586,161.05) .. (586,150) .. controls (586,138.95) and (591.01,130) .. (597.2,130) -- cycle ;
%Straight Lines [id:da41948477957491315] 
\draw    (525,130) -- (525,103) ;
\draw [shift={(525,100)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da46765068394916465] 
\draw    (165,60) .. controls (210.31,35.87) and (427.35,39.39) .. (481.63,39.98) ;
\draw [shift={(484,40)}, rotate = 180.57] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da049202105979806565] 
\draw    (200,150) -- (247,150) ;
\draw [shift={(250,150)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da7332174922286125] 
\draw    (200,80) .. controls (248.73,80.97) and (282.57,103.35) .. (284.87,127.38) ;
\draw [shift={(285,130)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da38567227747957566] 
\draw    (320,150) .. controls (322.48,89.11) and (411.69,52.24) .. (481.88,50.06) ;
\draw [shift={(484,50)}, rotate = 178.78] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da12633093416573238] 
\draw    (320,150) -- (367,150) ;
\draw [shift={(370,150)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da11079438746727421] 
\draw    (405,130) .. controls (407.48,69.11) and (413.38,61.65) .. (481.9,60.05) ;
\draw [shift={(484,60)}, rotate = 178.78] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da49470446058307094] 
\draw    (440,150) -- (487,150) ;
\draw [shift={(490,150)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da6567932941119186] 
\draw    (566,61) .. controls (608.41,61) and (624.68,89.04) .. (625.47,127.06) ;
\draw [shift={(625.5,130)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da9830868420918312] 
\draw    (566.5,239) .. controls (609.62,239) and (623.45,215.47) .. (624.92,173.12) ;
\draw [shift={(625,170.5)}, rotate = 91.3] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Flowchart: Decision [id:dp32523602671331253] 
\draw   (42,200) -- (77,220) -- (42,240) -- (7,220) -- cycle ;
%Straight Lines [id:da777987600567184] 
\draw    (42,170) -- (42,197) ;
\draw [shift={(42,200)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Flowchart: Process [id:dp5469673646929455] 
\draw   (130,200) -- (210,200) -- (210,270) -- (130,270) -- cycle ;
%Straight Lines [id:da900362014660893] 
\draw    (165,200) -- (165,173) ;
\draw [shift={(165,170)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da4881612495198385] 
\draw    (77,220) .. controls (78.89,177.47) and (109.36,152.81) .. (127.05,150.23) ;
\draw [shift={(130,150)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

% Text Node
\draw (24,142) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize Start}};
% Text Node
\draw (134.5,143.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\scriptsize \#Banks $\displaystyle  >n$?}};
% Text Node
\draw (139,112) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize yes}};
% Text Node
\draw (211,132) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize no}};
% Text Node
\draw (132,73.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\scriptsize \#data $\displaystyle  >\ k$?}};
% Text Node
\draw (255.5,143) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\scriptsize MPC circuit}};
% Text Node
\draw (376.5,142.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize detection}};
% Text Node
\draw (496,142) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize Accuracy}};
% Text Node
\draw (490.5,213) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{45.33pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize Orchestrate}\\{\footnotesize MPC}
\end{center}

\end{minipage}};
% Text Node
\draw (490,41.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{45.33pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize Orchestrate}\\{\footnotesize FL}
\end{center}

\end{minipage}};
% Text Node
\draw (587,132) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\scriptsize Output to FI}\\{\scriptsize or authorities}};
% Text Node
\draw (221.5,85) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize no}};
% Text Node
\draw (179,32) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize yes}};
% Text Node
\draw (328,77) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize hard}};
% Text Node
\draw (331,132) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize easy}};
% Text Node
\draw (373.5,96) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize online}};
% Text Node
\draw (451,132) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize offline}};
% Text Node
\draw (529,112.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize confidence}};
% Text Node
\draw (527,173) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize Best}};
% Text Node
\draw (15.5,212) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize Adversary}};
% Text Node
\draw (59,242) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize Malicious}};
% Text Node
\draw (151,212) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{26.29pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize Prove }\\{\footnotesize in ZK}
\end{center}

\end{minipage}};
% Text Node
\draw (85,182) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\footnotesize semi-honest}};


\end{tikzpicture}


==> payment-model.tex <==
\section{CBDC System Model and Features}

%\textbf{Model and needed properties:}
%\begin{itemize}
%	\item Payment system properties 
%	\begin{itemize}
%		\item Topology
%		\item System entities
%		\item Access permissions
%		\item Ledger/database properties
%	\end{itemize}
%	\item Basic checks
%\begin{itemize}
%	\item Authenticity
%	\item Balance
%	\item Non-negative assets
%\end{itemize}
%	\end{itemize}
%
%\noindent\textbf{Desired features:}
%	\begin{itemize}
%	\item Privacy properties
%	\begin{itemize}
%		\item Confidentiality
%		\item Anonymity
%	\end{itemize}
%
%	\item Accountability (proactive)
%	\begin{itemize}
%	\item Blacklist checks
%	\item Transaction characteristics
%	\end{itemize}
%	\item Auditability (reactive)
%	\begin{itemize}
%	\item Patterns
%	\item Targeted audits
%	\end{itemize}
%
%\end{itemize}



%Reactive checks' output might not be definitive, but with some confidence factor lower than 1 (i.e. cryptographic vs. machine-learning solutions).
